Traceable Automatic Feature Transformation via Cascading Actor-Critic Agents

Feature transformation for AI is an essential task to boost the effectiveness and interpretability of machine learning (ML). Feature transformation aims to transform original data to identify an optimal feature space that enhances the performances of a downstream ML model. Existing studies either combines preprocessing, feature selection, and generation skills to empirically transform data, or automate feature transformation by machine intelligence, such as reinforcement learning. However, existing studies suffer from: 1) high-dimensional non-discriminative feature space; 2) inability to represent complex situational states; 3) inefficiency in integrating local and global feature information. To fill the research gap, we formulate the feature transformation task as an iterative, nested process of feature generation and selection, where feature generation is to generate and add new features based on original features, and feature selection is to remove redundant features to control the size of feature space. Finally, we present extensive experiments and case studies to illustrate 24.7\% improvements in F1 scores compared with SOTAs and robustness in high-dimensional data.

==> 4.method.old.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{fig/model_overall.pdf}
    \vspace{-0.2cm}
    \captionsetup{justification=centering}
    \vspace{-0.33cm}
    \caption{An overview of the proposed framework AFG. (1) \textit{Feature Space Clustering} clustering the input feature. (2) \textit{Feature Set (Group) and Operation State Representation Methods} extract the latent information (state) within the overall features, selected feature clusters, and selected operation. (3) \textit{Cascading Actor-Critic Agents} make decision depends on state to construct the mathematical transformation in current step. (4) \textit{Dataset Evaluator} evaluates the generated features to obtain the overall reward. We use $s_{(\cdot)}$ to represent a state of overall feature, a feature cluster or an operation.
    }
    \vspace{-0.45cm}
\label{model_overall}
\end{figure*}

\subsection{Model Overview}
We demonstrate the overview of \ul{A}ctor-Critic based \ul{F}eature \ul{G}eneration (AFG) model in Figure~\ref{model_overall}. We give a detailed description of each component in the following sections.

\vspace{-0.3cm}

\subsection{Feature Space Clustering}
As a pre-step to facilitate the model performance, we propose the feature space clustering component. In the following sections, we first introduce three functions to measure the relevance of two clusters. Then, we describe the Features-Group Clustering (FG-Clustering) methods.

\noindent\textbf{Features-Group Distance Functions:}
We propose this function to measure the similarity between two clusters of features. Suppose we have two clusters $c_i$ and $c_j$, the formal definition of features-group distance function is give by:
% \begin{equation}
% \begin{aligned}
%   \small
%     \label{dis}
%     d_{m}(c_i, c_j)= 
%     \frac{1}{|c_i|\cdot|c_j|}
%     \sum_{f_i\in c_i}\sum_{f_j\in c_j}
%     \frac{|\text{dis}(f_i,y)-\text{dis}(f_j,y)|}{\text{dis}(f_i,f_j)+\epsilon},  
% \end{aligned}
% \vspace{-0.2cm}
% \end{equation}
\begin{equation}
\begin{aligned}
  \small
    \label{dis}
    d_{m}(c_i, c_j)= 
    \frac{1}{|c_i|\cdot|c_j|}
    \sum_{f_i\in c_i}\sum_{f_j\in c_j}
    |\text{dis}(f_i,f_j)|,  
\end{aligned}
\vspace{-0.2cm}
\end{equation}
where $dis(\cdot)$ is a pair-wise distance function (e.g., the euclidean distance, cosine similarity, etc). In Equation~\ref{dis}, the numerator  (i.e., $|\text{dis}(f_i,y)-\text{dis}(f_j,y)|$) aims to quantify the relevancy between the feature columns and the target. 
The denominator (i.e., $\text{dis}(f_i,f_j)+\epsilon$) quantifies the redundancy between $f_i$ and $f_j$. The $\epsilon$ is a small constant to avoid the divide by zero error. If the numerator is small, $f_i$ and $f_j$ should have a similar influence on the classification of $y$. And, when the denominator is big, it represents $f_i$ and $f_j$ share more information. Both make the function gives these two columns of feature with a smaller distance. 

\iffalse
\noindent1) \textit{Euclidean Distance Based:} The first method trying to measure the similarity between two clusters by the euclidean distance. We assume that the cluster method should merge two clusters of features with a smallest absolute value of the numerical difference into one cluster. The euclidean distance function between two clusters can be defined as:
\vspace{-0.2cm}
\begin{equation}
\begin{aligned}
  \small
    % \label{mi_dis}
    d_{e}(c_i, c_j)= 
    \frac{1}{|c_i|\cdot|c_j|}\sum_{f_i\in c_i}\sum_{f_j\in c_j}
    \sqrt{\sum(f_i-f_j)^2},  
\end{aligned}
\vspace{-0.2cm}
\end{equation}

\noindent2) \textit{Cosine Similarity Based:} Another idea to measure the distance is to utilize the cosine similarity. Compared to the euclidean distance, the cosine similarity will be more sensitive to the feature columns with little numeric difference. The definition of cosine similarity based features-group distance functions is defined by:
% In some cases, when two features are varied in numeric but similar in purpose (e.g., two columns of features describe the same length but one in meter and the other in millimeter), this distance function help the FG-cluster algorithm to group them. 
\vspace{-0.2cm}
\begin{equation}
\begin{aligned}
  \small
    % \label{mi_dis}
    d_{c}(&c_i, c_j)= 
    \frac{1}{|c_i|\cdot|c_j|}\sum_{f_i\in c_i}\sum_{f_j\in c_j}
    (1 - \frac{f_i\cdot f_j}{||f_i||\cdot||f_j||}),  
\end{aligned}
\vspace{-0.2cm}
\end{equation}

\noindent3) \textit{Mutual Information Based:} The last method is to utilize the mutual information (MI) between the column of the feature and its related label. We assume that two clusters with similar relevance to the target should have a smaller distance. Thereby, the MI based features-group distance functions  $d_{m}(\cdot)$ is defined as:
% \vspace{-0.2cm}
\begin{equation}
\begin{aligned}
  \small
    \label{mi_dis}
    d_{m}(c_i, c_j)= 
    \frac{1}{|c_i|\cdot|c_j|}
    \sum_{f_i\in c_i}\sum_{f_j\in c_j}
    \frac{|\text{MI}(f_i,y)-\text{MI}(f_j,y)|}{\text{MI}(f_i,f_j)+\epsilon},  
\end{aligned}
\vspace{-0.2cm}
\end{equation}
where the $\text{MI}(\cdot)$ is the function to obtain the mutual information between two vectors. $|c_i|$ and $|c_j|$ are the total number of two clusters. 

In Equation~\ref{mi_dis}, the numerator  (i.e., $|\text{MI}(f_i,y)-\text{MI}(f_j,y)|$) aims to quantify the relevancy between the feature columns and the target. 
The denominator (i.e., $\text{MI}(f_i,f_j)+\epsilon$) quantifies the redundancy between $f_i$ and $f_j$. The $\epsilon$ is a small constant to avoid the divide by zero error. If the numerator is small, $f_i$ and $f_j$ should have a similar influence on the classification of $y$. And, when the denominator is big, it represents $f_i$ and $f_j$ share more information. Both make the function gives these two columns of feature with a smaller distance. 
\fi


\noindent\textbf{FG-Clustering:}
Due to the number of feature columns varying during feature generation. Therefore, it is not appropriate to use K-means or density based methods. Inspired by agglomerative clustering, given a feature set $\mathcal{F}$, we propose the FG-Clustering in two steps. Specifically,  
\ul{\textit{Step-1}}:  
we initialize each column in $\mathcal{F}$ as a cluster. \ul{\textit{Step-2}}:  
we use the features-group distance function (i.e., $d_e(\cdot)$, $d_c(\cdot)$, or $d_m(\cdot)$) to obtain the distance between any two feature clusters. Then, we merge the two closest clusters to generate a new cluster and remove the former ones. We repeat this step until the smallest distance between any two clusters reaches a certain threshold. 
\ul{\textit{Output}}: We cluster the columns of $\mathcal{F}$ and form the cluster set $C=\{c_i\}_{i=1}^{|C|}$.


\vspace{-0.3cm}
\subsection{Feature State Representation}
To describe the state of feature space, our intuitive idea is to propose a function $\mathcal{R}(\cdot) \to s_{(\cdot)}$. The output $s_{(\cdot)}$ is a fixed-size vector to represent the state of a length-variable input feature. 
In this section, we introduce three methods for different aspects of feature space.  
To simplify the description, in the following parts, suppose given the feature set $\mathcal{F}\in \mathbb{R}^{M\times N}$, where $M$ is the number of the total samples, and $N$ is the number of feature columns. 

% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/state_ds.pdf}
%     \vspace{-0.2cm}
%     \captionsetup{justification=centering}
%     \vspace{-0.33cm}
%     \caption{The process to obtain the state representation by using statistic information of features.  
%     }
%     \vspace{-0.25cm}
%     \label{fig:ds}
% \end{figure}

\noindent\textbf{Statistic Information (si):} The first idea is to utilize the statistic information (\textit{i.e.} count, standard deviation, minimum, maximum, first, second, and third quartile) of the input feature cluster.
% Figure~\ref{fig:ds} shows its calculation process in three steps.
Specifically, \ul{\textit{Step-1}}: We calculate the descriptive statistics matrix  of $\mathcal{F}$ column by column. \ul{\textit{Step-2}}: We calculate the descriptive statistics of the outcome matrix of the previous step row by row to obtain the meta descriptive statistics matrix that shape is $\mathbb{R}^{7\times 7}$.\ul{\textit{Step-3}}: We obtain the feature-feature's state representation $\mathcal{R}_{si}(\mathcal{F})\in \mathbb{R}^{1\times 49}$ by flatting the descriptive matrix from the former step.


% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/state_ae.pdf}
%     \vspace{-0.2cm}
%     \captionsetup{justification=centering}
%     \vspace{-0.33cm}
%     \caption{The process to obtain the state representation by using latent information from autoencoder.  
%     }
%     \vspace{-0.25cm}
%     \label{fig:ae}
% \end{figure}

\noindent\textbf{Autoencoder (ae):}
Another idea is to utilize autoencoder to convert  the feature set $\mathcal{F}$ into a latent embedding vector and regard it as the state representation.
% Figure~\ref{fig:ae} shows the calculation process in three steps.
Specifically, \ul{\textit{Step-1:}} We apply an autoencoder to transform each column of $\mathcal{F}$ into a latent matrix $Z \in \mathbb{R}^{k\times N}$, where $k$ is the dimension of the latent representation of each column.
\ul{\textit{Step-2:}} We apply another autoencoder to transform each row of $Z$ in to another matrix $Z' \in \mathbb{R}^{k\times d}$, where $d$ is the dimension of the latent representation of each row.
\ul{\textit{Step-3:}} We obtain the state representation vector $\mathcal{R}_{ae}(\mathcal{F}) \in \mathbb{R}^{1 \times kd}$ by flattening the matrix $Z'$.


% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/state_gae.pdf}
%     \vspace{-0.2cm}
%     \captionsetup{justification=centering}
%     \vspace{-0.33cm}
%     \caption{The process to obtain the state representation by using graph autoencoder. 
%     }
%     \vspace{-0.55cm}
%     \label{fig:cg}
% \end{figure}
\noindent\textbf{Graph Autoencoder (gae):}
The last idea is to train a graph autoencoder~\cite{https://doi.org/10.48550/arxiv.1611.07308} to reconstruct the correlation graph between each column of features. 
% Figure~\ref{fig:cg} shows the calculation process.
Specifically, 
\ul{\textit{Step-1}}: We build a complete correlation graph $\mathcal{G}$ by calculating the similarity matrix between each pair of feature columns.
The adjacency matrix of $\mathcal{G}$ is $\mathcal{A} \in \mathbb{R}^{N\times N}$, where a node is a feature column in $\mathcal{F}$ and an edge reflects the similarity between two nodes.
\ul{\textit{Step-2}}: We adopt a one-layer GCN~\cite{kipf2016semi} to aggregate a  enhanced feature embeddings $Z\in \mathbb{R}^{N\times k}$ based on $\mathcal{A}$, where $k$ is the dimension of latent embedding. The calculation process is defined as:
$
Z = ReLU(\mathbf{D}^{-\frac{1}{2}}\mathcal{A}\mathbf{D}^{-\frac{1}{2}}\mathcal{F}^{\top}\mathbf{W}),
$
where $\mathbf{D}$ is the diagonal node degree matrix of $\mathcal{A}$, and $\mathbf{W}\in\mathbb{R}^{N\times k}$ is the weight matrix of the GCN.
\ul{\textit{Step-3}}: 
We average $Z$ column-wisely to obtain the state representation $\mathcal{R}_{gae}(\mathcal{F}) \in \mathbb{R}^{1\times k}$. 

To obtain the state representation of operation $o \in \mathcal{O}$, we use a one-hot lookup table, denoted as $\mathcal{R}_{o}(o)$. 
\vspace{-0.2cm}
\subsection{Dataset Evaluator} We introduce two utility metrics from the supervised and unsupervised perspectives to evaluate the generated features and obtain the reward for cascading agents.

\noindent\textbf{Downstream Task:} 
We utilize the improvement of a downstream task (e.g., regression, classification) as the metric. In detail, we use a random forest based method and task-specific indicator $P_A(\mathcal{F}, y)$ (e.g., 1-RAE, Precision, Recall, F1) as the method and utility metric of a feature set. 

\noindent\textbf{Feature Quality:}
We should also consider the generated feature quality to evaluate the dataset. In detail, we hope the generated features contain less redundancy and more relevance to the target. Thus, we apply mutual information to measure the feature quality:
\begin{equation}
\small
    U(\mathcal{F}|y) = -\frac{1}{|\mathcal{F}|^2}\sum_{f_i, f_j \in \mathcal{F}} \text{MI}(f_i, f_j) + \frac{1}{|\mathcal{F}|}\sum_{f\in \mathcal{F}}\text{MI}(f,y),
\end{equation}
where $f_i, f_j, f$ are features in $\mathcal{F}$ and $|\mathcal{F}|$ is the size of the feature set $\mathcal{F}$.


\vspace{-0.2cm}
\subsection{Cascading Agents}
We model the process to choose one or two cluster(s) and the most suitable operation as three markov decision processes (MDPs) and develop three agents. 
% Here, given the input feature set $\mathcal{F}$, after the progress, the cascading agents will generate the feature set $\mathcal{F}'$ for the next step. 
% such as head cluster select agent ($\text{Agent}_h$), operation select agent ($\text{Agent}_o$), and tail cluster select agent ($\text{Agent}_t$), respectively. 
% \iffalse
% \noindent\textbf{Actor-critic agent:}
% We consider an off-policy actor-critic approach~\cite{ddpg, lillicrap2015continuous} to construct robust cascading agents. For each agent, we construct two pairs of policy networks (Actor) and value networks (Critic). 

% \noindent\ul{\textit{Actor}}: The Actor $\mu$ and its target network $\beta$ are with the same architecture and will take the current state $s$ and output the probability distribution of each action. Both of them will initial with same parameter.

% \noindent\ul{\textit{Critic}}: The Critic network $V_{\mu}$ and its target network $V_{\beta}$  are also with same architecture. They will evaluate the current state and output the current value. 

% \noindent\ul{\textit{Advantage}}: Given current state $s$ and the state of generated feature $s'$,
% \fi

\noindent\textbf{Head Agent:}
The head cluster select agent $\text{Agent}_h$ will consider two fact: 1) the overall state $s_f$ of input feature $\mathcal{F}$; 2) the state $s_{c_i}$ of cluster $c_i$. 

\noindent\ul{\textit{Actor}}: The formal definition of the actor network is:
\vspace{-0.1cm}
\begin{equation}
    c_h \sim \pi_h(\left[s_f\oplus s_{c_i} \right]_{i=1}^{|C|}; \theta_{\pi_h}),
\vspace{-0.1cm}
\end{equation}
where $\pi_h(\cdot)$ is two layer feed-forward network with a softmax activation and will output a probability distribution of each action. $\theta_{\pi_h}$ is the learnable parameter. $\oplus$ operation will element-wise concanecat the overall state and the specific cluster state. We use $\sim$ to represent we sample the cluster $c_h$ from the output distribution of policy network $\pi_h(\cdot)$.

\noindent\ul{\textit{Critic}}: The critic will consider the overall state $s_f$, defined as:
    $v_h = V_h(s_f; \theta_{v_h})$,
where $V_h(\cdot)$ is two layers feed-forward networks with parameter $\theta_{v_h}$. The output $v_h$ is the value of the state. 


\noindent\ul{\textit{Reward}}: The reward of $\text{Agent}_h$ is the generated feature quality, denoted by: $r_h = U(\mathcal{F}'|y)$.

\noindent\textbf{Operation Agent:} $\text{Agent}_o$ will pick an operation $o \in \mathcal{O}$ according to the state $s_{h}$ of the head cluster. 

\noindent\ul{\textit{Actor}}:
The definition of the actor network is:
\vspace{-0.2cm}
\begin{equation}
    op \sim \pi_o(s_{h}; \theta_{\pi_o}),
    \vspace{-0.2cm}
\end{equation}
where $\pi_o(\cdot)$ is two layers feed-forward networks with a softmax activation. $\theta_{\pi_o}$ is a learnable parameter. $s_{h}$ is the state representation of the selected head cluster $c_h$. The agent will sample an operation $op$ from the output distribution of  $\pi_o(s_{h})$.

\noindent\ul{\textit{Critic}}: We adopt two layers  feed-forward networks with parameter $\theta_{v_t}$, denoted as $v_o = V_o(s_{h}; \theta_{v_t})$, to evaluate the value of the $s_{h}$.  

\noindent\ul{\textit{Reward}}: The reward of $\text{Agent}_o$ will regard the generated feature quality and downstream task performance, denoted by: $r_o = U(\mathcal{F}'|y) + P_A(\mathcal{F}', y) - P_A(\mathcal{F}, y)$.

\noindent\textbf{Tail Agent:}
For the tail cluster select agent, we regard the overall state $s_f$, the state of head cluster $s_{h}$, the state of operation $s_o$, and each cluster's state $\{s_{c_i}\}_{i=1}^{|C|}$ to decide the tail cluster selection.

\noindent\ul{\textit{Actor}}: The formal definition of the policy network is:
\vspace{-0.2cm}
\begin{equation}
   c_t \sim \pi_t(\left[s_f\oplus s_o\oplus s_h\oplus s_{c_i} \right]_{i=1}^{|C|};\theta_{\pi_t}),
   \vspace{-0.2cm}
\end{equation}
where $\pi_t(\cdot)$ is two layers feed-forward networks with softmax activation. $\theta_{\pi_t}$ is the parameter. During the decision-making, the agent will sample the tail cluster $c_t$ from the output.

\noindent\ul{\textit{Critic}}: The critic will consider the overall state $s_f$, head cluster state $s_h$, chosen operation state $s_o$, defined as:
    $v_t = V_t(s_f \oplus s_h \oplus s_o; \theta_{v_t})$,
where $V_t(\cdot)$ is two layer feed-forward networks with parameter $\theta_{v_t}$. $v_t$ is the value of the current state. 


\noindent\ul{\textit{Reward}}: The reward of $\text{Agent}_t$ is the generated feature quality, denoted by: $r_t = U(\mathcal{F}'|y)$.


\vspace{-0.2cm}
\subsection{Model Training}
% Due to each agent taking on different responsibilities and interdependent, we design a unique reward for each agent. We hope the head agent and tail agent can select a feature cluster that can generate little redundancy feature, and the operation agent can choose an action that is most suitable for the downstream task and also can generate good-quality features.
Suppose that during the exploration, for each agent, we can obtain the memory as $\mathcal{M} = (a, s, s', r)$, where $a$ is the selected action (e.g., $c_h$ for $\text{Agent}_h$, $op$ for  $\text{Agent}_o$, and $c_t$ for $\text{Agent}_t$). $s$ and $s'$ is the input state for current step and next step. $r$ is the reward for adopt action $a$.  
We minimize the temporal difference error $L$, given by:
\vspace{-0.1cm}
\begin{equation}
\begin{aligned}
  \label{Q_update}
    \delta =& r + \gamma V(s'; \theta_v) - V(s; \theta_v)\\
    L(\mathcal{M}; \theta_\pi, \theta_v)& = log\pi (a|s;\theta_\pi) * \delta + \beta H(\pi (s; \theta_\pi))
    \vspace{-0.1cm}
\end{aligned}
\end{equation}
where $\gamma \in [0\sim 1]$ is the discounted factor.  $\delta$ is the advantage value. $H(\cdot)$ is an entropy regularization term. We use $\beta$ to controls the strength of the $H$. 

During the model exploration, we obtain the memories $\mathcal{M}_h$, $\mathcal{M}_o$, $\mathcal{M}_t$ for the cascading agents. Thus, we can formulate the loss function for cascading agent as:
\begin{equation}
\begin{aligned}
\small
\mathcal{L} = \sum_{i=\{h,o,t\}} L(\mathcal{M}_i; \theta_{\pi_i}, \theta_{v_i})
\end{aligned}
\end{equation}
\vspace{-0.7cm}


==> 8.ackownledgement.tex <==
This work is partially supported by IIS-2152030, IIS-2045567, and IIS-2006889.

==> tables/dataset.tex <==
\begin{table}[!htbp]
\centering
\caption{The description of the dataset. `C' for the Classification task, `R' for the Regression task, and `D' for the Outlier Detection task.}
\label{dataset}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Dataset Name            & Source   & Task & Samples & Features & Data Std.\\
\midrule
PimaIndian         & UCIrvine & C   & 768     & 8 &  High \\
SVMGuide3  & LibSVM & C & 1243 & 21 & Low\\
Amazon Employee    & Kaggle   & C   & 32769   & 9 & Very High   \\
German Credit      & UCIrvine & C   & 1001    & 24  & High \\
Wine Quality Red   & UCIrvine & C   & 999     & 12  & High  \\
Wine Quality White & UCIrvine & C   & 4900    & 12   & Low \\\midrule
Openml\_618        & OpenML   & R   & 1000    & 50  & Very Low \\
Openml\_589        & OpenML   & R   & 1000    & 25  & Very Low  \\
Openml\_616        & OpenML   & R   & 500     & 50 & Very Low   \\
Openml\_607        & OpenML   & R   & 1000    & 50  & Very Low  \\
Openml\_620        & OpenML   & R   & 1000    & 25  & Very Low  \\
Openml\_637        & OpenML   & R   & 500     & 50   & Very Low \\
Openml\_586       & OpenML   & R   & 1000    & 25  & Very Low \\\midrule
WBC & UCIrvine   & D   & 278    & 30 & Very Low\\
Mammography        & OpenML   & D   & 11183    & 6 & Very Low  \\
Thyroid        & UCIrvine   & D   & 3772    & 6  & Low  \\
SMTP        & UCIrvine   & D   & 95156    & 3 & High\\
\bottomrule
\end{tabular}}
\end{table}
